What Are "X-Shaped" Radio Sources Telling Us? II. Properties of a Sample of 87

In an earlier paper we presented Jansky Very Large Array multi-frequency, multi-array continuum imaging of a unique sample of low axial-ratio radio galaxies. In this paper, the second in the series, we examine the images to know the phenomenology of how the off-axis emission relates to the main radio source. Inversion symmetric offset emission appears to be bimodal and to originate from one of two strategic locations: outer ends of radio lobes (Outer-deviation) or from inner ends (Inner-deviation). The latter sources are almost always associated with edge-brightened sources. With S- and Z-shaped sources being a subset of Outer-deviation sources this class lends itself naturally to explanations involving black hole axis precession. Our data allow us to present a plausible model for the more enigmatic Inner-deviation sources with impressive wings; as for outer-deviation sources these too require black hole axis shifts although also requiring plasma backflows into relic channels. Evolution in morphology over time relates the variety in structures in inner-deviation sources including XRGs. With features such as non-collinearities, central inner-S "spine", corresponding lobe emission peaks, double and protruding hotspots not uncommon, black hole axis precession, drifts, or flips could be active in significant fraction of radio sources with prominent off-axis emission. At least 4\% of radio galaxies appear to undergo black hole axis rotation. Quasars offer a key signature to recognize rotating axes. With rich haul of sources that have likely undergone axis rotation our work shows the usefulness of low axial-ratio sources to pursue searches for binary supermassive black holes.

==> Table3.tex <==
%rejects.tex 15feb2017 ls & dr 16feb2017 dr

%\begin{landscape}

\begin{deluxetable}{cllll}

\tablecaption{Rejected Sources \label{tab:reject}}

\tablecolumns{5}

%\tablehead{ \colhead{Source}  &  \colhead{Paper I}  &  \colhead{JVLA: Band/Array, Date} }


\tablehead{ \colhead{Name} & %\colhead{RA} & \colhead{Dec} & 
 \colhead{z/ID?} & \colhead{Morphology} & \colhead{ID? Core?} & \colhead{Notes}  }
\startdata
J0033$-$0149 & %00 33 02.41  & $-$01 49 56.6 &
0.1301,  Yes & WAT? & Yes,  Yes &  \tablenotemark{a} \\
J0049+0059  & %00 49 39.45  & +00 59 53.8  &
 0.3044,  ? & confused & Confused src    &  \tablenotemark{b} \\
J0143$-$0119 & %01 43 16.75  & $-$01 19 00.8  & 
0.520,  yes & FR-I,  HT? & Yes,  Yes &  \tablenotemark{c} \\
J0821+2922 & %08 21 49.60  & +29 22 44.4  &  
 (0.332),  Yes? & lobe,  3.7\arcmin? & Yes?,  Yes? &  \tablenotemark{d} \\
J1111+4050 & %11 11 39.74 & 40 50 24.1 &
0.0737, \dots & HT & \dots & \tablenotemark{e}  \\
J1128+1919 & %11 28 37.7 & +19 19 57 &
 \dots, \dots & HT/confused?  &   \dots  &   \tablenotemark{f} \\
J1201$-$0703 & %12 01 25.76  & $-$07 03 11.0  & 
??,  Yes & WAT & 16.4,  bright! &  \tablenotemark{g}  \\
J1210+1121 & %12 10 11.99  & +11 21 02.7  & 
0.1963 ,  Yes & WAT? & 16.6,  bright & \tablenotemark{h} \\
J1227+2155 & %12 27 49.45  & +21 55 19.6  & 
0.459 ,  Yes & FR-II,  confused  & Yes?  yes1/yes1 &  \tablenotemark{i}  \\
J1330$-$0206  & %13 30 10.32  & $-$02 06 18.0 &
 0.0866,   Yes & WAT? & 15.5,  bright!  &  \tablenotemark{j} \\
J1339$-$0016 & %13 39 34.23  & $-$00 16 35.5 & 
0.1452,  Yes & WAT? & 15.9,  bright! &  \tablenotemark{k} \\\
J1522+4527 & %15 22 13.1  & +45 27 57  &
 (0.450),  No & ? 53\arcsec & No,  ? &   \tablenotemark{l}\\
J2226+0125 & %22 26 45.6  & +01 25 11  & 
   (0.216),  Yes & galaxy group & \dots &  \tablenotemark{m} \\
\enddata

\tablenotetext{a}{Complex structure. WAT projected? CD host. Dense group of galaxies.}
\tablenotetext{b}{Complex. Superposed sources?} 
\tablenotetext{c}{NS wingsize $=$ 540~kpc! Badly need high resolution maps to see if jets are associated with central core.} 
\tablenotetext{d}{DR12-photoz. SW lobe of much larger ~3.5\arcmin FR-II. Very asymmetric lobes. Core seen. See Paper-1 map!} 
\tablenotetext{e}{Head-Tail source.}
\tablenotetext{f}{Head-Tail source with core and ID at extreme south.} 
\tablenotetext{g}{Not in DR12! The only source with lobes deviated to the same side. Not to be considered.}
\tablenotetext{h}{ \ Likely severely projected. Absorption spectrum!}
\tablenotetext{i}{DR12. not observed yet with evla. Present in Paper-1. Cluster relic??}
\tablenotetext{j}{ \ Likely to be a WAT?} 
\tablenotetext{k}{ \ Likely a WAT. Many galaxies in vicinity of host.} 
\tablenotetext{l}{DR12. Nature of src unclear. Given ID is wrong--no ID for this src.  Both ``wings'' are on same side. No host though.} 
\tablenotetext{m}{DR12. No spectrum. Two galaxies seen in radio.}

\end{deluxetable}

%\end{landscape}

